Challenges and Opportunities to Enable Large-Scale Computing via Heterogeneous Chiplets

Fast-evolving artificial intelligence (AI) algorithms such as large language models have been driving the ever-increasing computing demands in today's data centers. Heterogeneous computing with domain-specific architectures (DSAs) brings many opportunities when scaling up and scaling out the computing system. In particular, heterogeneous chiplet architecture is favored to keep scaling up and scaling out the system as well as to reduce the design complexity and the cost stemming from the traditional monolithic chip design. However, how to interconnect computing resources and orchestrate heterogeneous chiplets is the key to success. In this paper, we first discuss the diversity and evolving demands of different AI workloads. We discuss how chiplet brings better cost efficiency and shorter time to market. Then we discuss the challenges in establishing chiplet interface standards, packaging, and security issues. We further discuss the software programming challenges in chiplet systems.

==> zz_9_standardizing.tex <==
%\section{Standardization in Heterogeneous Chiplets System}
%a) Software APIs \\
% Which standard should be followed by both vendors and communities to provide usability and generality
%b) Communication Protocol Standards\\
%c) Package Standards
